Effectiveness of Structural Restrictions for Hybrid CSPs

Constraint Satisfaction Problem (CSP) is a fundamental algorithmic problem that appears in many areas of Computer Science. It can be equivalently stated as computing a homomorphism $\mbox{$\bR \rightarrow \bGamma$}$ between two relational structures, e.g.\ between two directed graphs. Analyzing its complexity has been a prominent research direction, especially for {\em fixed template CSPs} in which the right side $\bGamma$ is fixed and the left side $\bR$ is unconstrained. Far fewer results are known for the {\em hybrid} setting that restricts both sides simultaneously. It assumes that $\bR$ belongs to a certain class of relational structures (called a {\em structural restriction} in this paper). We study which structural restrictions are {\em effective}, i.e.\ there exists a fixed template $\bGamma$ (from a certain class of languages) for which the problem is tractable when $\bR$ is restricted, and NP-hard otherwise. We provide a characterization for structural restrictions that are {\em closed under inverse homomorphisms}. The criterion is based on the {\em chromatic number} of a relational structure defined in this paper; it generalizes the standard chromatic number of a graph. As our main tool, we use the algebraic machinery developed for fixed template CSPs. To apply it to our case, we introduce a new construction called a "lifted language." We also give a characterization for structural restrictions corresponding to minor-closed families of graphs, extend results to certain Valued CSPs (namely conservative valued languages), and state implications for CSPs with ordered variables, (valued) CSPs on structures with large girth, and for the maximum weight independent set problem on some restricted families of graphs including graphs with large girth.

==> implications-short.tex <==
\subsection{Implications of Theorems \ref{coloreffective}, \ref{bjkineffective} and \ref{vcspconsineff}}
\myparagraph{Ordered CSP}
%
One natural structural restriction to fixed template CSP is to introduce ordering of variables and request the constraints to respect the ordering.

\begin{definition} We call a relational structure $(V, r_1, \dots, r_k)$ \emph{ordered} if, after some identification of $V$ with $[n]$ for $n =|V|$, whenever $(v_1, \dots, v_{\ar(r_j)}) \in r_j$ for some $j = 1, \dots, k$, then $v_1 < \dots < v_{\ar(r_j)}$.
\end{definition}

\begin{theorem} Let $\mathcal{H}$ be the set of all ordered relational structures of some fixed signature.
Such structural restriction  $\mathcal{H}$ is ineffective for BJK languages and for conservative valued languages.
\end{theorem}

\ignore{
\begin{proof} It suffices to show that preconditions of Theorems \ref{bjkineffective} and \ref{vcspconsineff} hold.
\begin{itemize}
\item $\mathcal{H}$ up-closed:

Let $\mathbf{R} = (V, r_1, \dots, r_k) \in \mathcal{H}$ and $\mathbf{R}' \to \mathbf{R}$ where $\mathbf{R}' = (V', r'_1, \dots, r'_k)$ and let $h \colon V' \to V$ be the homomorphism. We may assume $V = [n]$. Let us define a partial order on $V'$ such that $v'_1 < v'_2$, if $h(v'_1) < h(v'_2)$. Extend this partial order arbitrarily to a total order on $[m]$ for $m = |V'|$ and identify $V'$ and $[m]$.

Now take $(v_1, \dots, v_{\ar(r'_j)}) \in r'_j$ for some $j = 1, \dots, k$ and since $(h(v_1), \dots, h(v_{\ar(r'_j)})) \in r_j$, we have $h(v_1) < \dots < h(v_{\ar(r'_j)})$ and thus also $v_1 < \dots < v_{\ar(r'_j)}$.

We just verified that $\mathbf{R}' \in \mathcal{H}$.

\item $\chi(\mathcal{H}) = \infty$:

Fix $n \in \mathbb{N}$. We will construct $\mathbf{R} \in \mathcal{H}$ that cannot be properly colored with $n$ colors. Let $m$ be the maximal arity of relations in $\mathcal{H}$. Let $\mathbf{R} = (V, r_1, \dots, r_k)$ where $V = [n(m-1)+1]$ and for $j = 1, \dots, k$ we set $(v_1, \dots, v_{\ar(r_j)}) \in r_j$ if and only if $v_1 < \dots < v_{\ar(r_j)}$.

Clearly, $\mathbf{R} \in \mathcal{H}$. Now for any coloring with $n$ colors some color (say red) appears at least $m$ times. Let $v_1 < \dots < v_m$ be red elements of $V$. But then the tuples $(v_1, \dots, v_{\ar(r_j)})$ are red for $j = 1, \dots, k$ and hence the coloring is improper. 
\item $\calH$ does not restrict unaries: this follows directly from definitions.
\end{itemize}
\end{proof}
}

This has an interesting consequence for graph homomorphism problems.

\begin{corollary} For the class of directed acyclic graphs $\mathcal{H}$, algebraic dichotomy conjecture implies that for every language $\bGamma=(D,\varrho)$ with a binary relation $\varrho$, $\CSP\Gamma$ is tractable if and only if $\cspo_{\calH}(\bGamma)$ is tractable.
\end{corollary}

\myparagraph{Minor-closed families of graphs}
%
It is known that a minor-closed family of undirected graphs has either bounded chromatic number or contains all graphs
(see~\cite[Lemma 2]{nesetril:minorclosed}). Using this result and Ramsey's Theorem, we can show the following.

\begin{theorem} Let the structural restriction $\mathcal{H}$ be a family of directed graphs such that the underlying family of undirected graphs is minor-closed. Then $\mathcal{H}$ is effective for BJK languages if and only if $\chi(\mathcal{H}) < \infty$.
\end{theorem}


%\myparagraph{Structures with large girth}
%
%As we said earlier, the family $\calH$ of graphs with girth at least $k$ is up-closed. Also, it is known to have unbounded chromatic number \cite{Erdös1966149}. However, the (unconditional) result that $\CSP\Gamma$ and $\cspo_\calH(\bGamma)$ have the same complexities for every $\Gamma$ is already known even in a more general setting:
%this has been shown in~\cite{Kun13}, for an appropriate definition of a girth of a relational structure.
%Namely, the ineffectiveness of restricting to high girth structures for arbitrary CSP was shown in~\cite{Kun13}
%(for an appropriate definition of a girth of a relational structure).
%
%The notion of a girth also exists for relational structures. The ineffectiveness of restricting to high girth structures for arbitrary CSP was shown in~\cite{Kun13}. 
%We extend this result to conservative VCSP languages.

%\begin{theorem} Let $\mathcal{H}$  be the set of all relational structures of some fixed signature whose girth is at least $k$, where $k\ge 2$ is some constant.
%The structural restriction $\calH$ is ineffective for the class of conservative valued languages.
%\end{theorem}






\myparagraph{Maximum Independent Set}
%
Although Theorem~\ref{vcspconsineff} is formulated for conservative languages, it also gives implications
for some optimization problems corresponding to non-conservative languages.
Namely, the following can be shown.
%
\begin{theorem} Let $\calG$ be a family of undirected graphs 
with $\chi(\calG) = \infty$ that is closed under inverse homomorphisms
(i.e.\ if $G,G'$ are undirected graphs such that $G\in\calG$ and $G'$ maps homomorphically to $G$
then $G'\in\calG$).
 Then
the {\sc max weight independent set} problem (with positive node weights) is NP-hard even when restricted to graphs in $\calG$.
\label{th:MWIS}
\end{theorem}





==> ineffproof.tex <==
For the entire section let $D$ be the domain $\Gamma = \{ \varrho_1, \varrho_2, \dots, \varrho_k \}$. Finally let $\mathcal{H} = \{ R_1, R_2, \dots \}$, where each $R_i = ( V_i, \varrho^{R_i}_1, \dots,  \varrho^{R_i}_k )$.


Since the restricted CSP cannot be harder, than the unrestricted one, it suffices to prove the following. If $CSP_\mathcal{H}(\Gamma)$ is tractable, then $CSP(\Gamma)$ is tractable.

The strategy is to construct a sequence of languages $\Gamma_\mathcal{H}^n$ for $n = 1,2, \dots$, which links, in terms of tractability, to both $CSP_\mathcal{H}(\Gamma)$ and $CSP(\Gamma)$.

In fact, we will prove the following.

\begin{proposition}\label{inherit_tract} Let $\mathcal{H}$ be an up-closed structural restriction and $\Gamma$ a constraint language. Then $CSP(\Gamma_\mathcal{H}^n)$ is polynomial-time reducible to If $CSP_\mathcal{H}(\Gamma)$ for every $n \in \mathbb{N}$.
\end{proposition}

For proving Theorems \ref{bjkineffective} and \ref{vcspconsineff} TODO motivation

\medskip


\subsection{Construction of $\Gamma_\mathcal{H}^n$}


Fix $n \in \mathbb{N}$. For $R_i \in \mathcal{H}$, we create a copy of the domain $D$ for each $v \in V_i$, denote it $D^{R_i}_{v}$ and define $$D^{R_i} = \bigcup_{v \in V_i} D^{R_i}_v.$$ We make sure the sets $D^{R_i}_v$ (taken over all pairs $(i,v)$) are pairwise disjoint and let $$D_n = \bigcup_{i \leq n} D^{R_i}.$$


For $i \leq n$ and $v \in V_i$ define a mapping $d^{R_i}_{v} \colon D \to D_n$ such that $d^{R_i}_{v}(a)$ is the copy of $a$ in $D^{R_i}_{v}$. Also for a tuple $a = (a_1, \dots, a_j) \in D^j$ define $d^{R_i}_{v}(a) = (d^{R_i}_{v}(a_1), \dots, d^{R_i}_{v}(a_j))$ and analogously for $b \in D_n$, define $d(b)$ the natural projection of $b$ on $D$ and for a tuple $b = (b_1, \dots, b_j)$, let $d(b) = (d(b_1), \dots, d(b_j))$.


Now for $\varrho_j \in \Gamma$, $R_i \in \mathcal{H}$, $i \leq n$, and $(v_1, \dots, v_{\ar(\varrho_j)}) \in V^{\ar(\varrho_j)}$ we will define a relation on $D_n$ of the same arity as $\varrho_j$, namely
$$(\varrho_j)^{R_i}_{v_1, \dots, v_{\ar(\varrho_j)}} = \{ (d^{R_i}_{v_1}(x_1), \dots, d^{R_i}_{v_{\ar(\varrho_j)}}(x_{\ar(\varrho_j)}) ) : (x_1, \dots, x_n) \in \varrho_j \}.  $$

Finally, we construct the sought language $\Gamma_{\mathcal{H}}^n$ on domain $D_n$ as follows

$$\Gamma_{\mathcal{H}}^n = \{(\varrho_j)^{R_i}_{v_1, \dots, v_{\ar(\varrho_j)}}: \varrho_j \in \Gamma, i \leq n, (v_1, \dots, v_{\ar(\varrho_j)}) \in \varrho^{R_i}_j \}. $$



\begin{lemma} \label{triv_lemma}
\begin{enumerate}
\item[(a)] If $(u_1, \dots, u_{\ar(\varrho_j)}) \in (\varrho_j)^{R_i}_{v_1, \dots, v_{\ar(\varrho_j)}}$, then $d(u_1, \dots, u_{\ar(\varrho_j)}) \in \varrho_j$.
\item[(b)] If $(u_1, \dots, u_{\ar(\varrho_j)}) \in \varrho_j$, then
$(d^{R_i}_{v_1}(u_1), \dots, d^{R_i}_{v_{\ar(\varrho_j)}}(u_{\ar(\varrho_j)})) \in (\varrho_j)^{R_i}_{v_1, \dots, v_{\ar(\varrho_j)}}.
$
\end{enumerate}


\end{lemma}

\subsection{Proof of Proposition \ref{inherit_tract}}

Fix $n \in \mathbb{N}$ and let $\mathcal{I}$ be an instance of $CSP(\Gamma_\mathcal{H}^n)$ with the set of variables $U$. We begin with a preprocessing step.

For $u \in U$ we look at all constraints containing it. Each of them restricts the admissible values of $u$ to a copy $D^{R_k}_v$ of $D$ for some $m \leq n$ and $v \in V_m$. In fact, this copy must be unique, otherwise the instance is automatically infeasible (and it can be checked in polynomial time).  Then for each $m \leq n$ and $v \in V_m$ we will denote the variables restricted to $D^{R_m}_v$ as $^{1}u^{R_m}_v$, $^{2}u^{R_m}_v$, \dots

We may assume every $u \in U$ was uniquely relabeled.

Next, observe that no constraint can contain simultaneously $^{i}u^{R_m}_v$ and $^{i'}u^{R_{m'}}_{v'}$ for $m \neq m'$. Therefore, $\mathcal{I}$ is a conjunction of independent instances $\mathcal{I'}_1$, \dots, $\mathcal{I'}_n$ such that each $\mathcal{I'}_m$ has the variable set
$$U'_m = \{ ^{i}u^{R_m}_v \colon v \in V_m, i \in \mathbb{N} \,\, \text{such that} \,\, ^{i}u^{R_m}_v \in U \}.$$

It suffices to decide satisfiability of $\mathcal{I}'_1$, \dots, $\mathcal{I}'_n$ independently. For this we will use tractability of $CSP_\mathcal{H}(\Gamma)$ and the up-closedness of $\mathcal{H}$.

Let us fix $m \leq n$ and simplify the notation a bit by writing $\mathcal{I'}$, $R = (V, \varrho^R_1, \dots, \varrho^R_k)$, $U'$, and $u^i_v$, instead of $\mathcal{I'}_m$, $R_m = (V_m, \varrho^{R_m}_1, \dots, \varrho^{R_m}_k)$, $U'_m$, and $^{i}u^{R_m}_v$.

As the next step we define an instance $\mathcal{I}_\Gamma$ of $CSP_\mathcal{H}(\Gamma)$ on the same set of variables $U'$. We specify the instance by providing the corresponding relational structure $R' = (U', r_1, \dots, r_k)$, where for $j = 1, \dots, k$ we set
$$r_j = \{(u_{v_1}^{i_1}, \dots, u_{v_{\ar(\varrho_j)}}^{i_{\ar(\varrho_j)}}) : (\varrho_j)^{R}_{v_1, \dots, v_{\ar(\varrho_j)}} \, \text{is applied to} \,\, (u_{v_1}^{i_1}, \dots, u_{v_{\ar(\varrho_j)}}^{i_{\ar(\varrho_j)}}) \,\, \text{in} \,\, \mathcal{I}'  \}.$$

Next we show that $R' \to R$. Since $R \in \mathcal{H}$ and $\mathcal{H}$ is up-closed, this will imply $R' \in \mathcal{H}$ and therefore $\mathcal{I}_\Gamma$ will indeed be an instance of $CSP_\mathcal{H}(\Gamma)$.

The mapping $h \colon U' \to V$ defined as $h(u^i_v) = v$ is the required homomorphism. Indeed for any $j = 1, \dots, k$, $(u_{v_1}^{i_1}, \dots, u_{v_{\ar(\varrho_j)}}^{i_{\ar(\varrho_j)}}) \in r_j$ implies $(\varrho_j)^{R}_{v_1, \dots, v_{\ar(\varrho_j)}} \in \Gamma^n_\mathcal{H}$ and thus $(v_1, \dots, v_{\ar(\varrho_j)}) \in \varrho_j^R$.

It remains to show that $\mathcal{I}_\Gamma$ is feasible if and only if $\mathcal{I'}$ is feasible. To this end, let $s \colon U' \to D_n$ be a solution to $\mathcal{I}'$. Then the mapping $s' \colon U' \to D$, $s'(u) = d(s(u))$ is a solution to $\mathcal{I}_\Gamma$. This follows from Lemma \ref{triv_lemma}(a). On the other hand if $t \colon U' \to D$ is a solution to $\mathcal{I}_\Gamma$, then the solution to $\mathcal{I}_\Gamma$ is given by the mapping $t' \colon U' \to D_n$ defined as $t'(u^i_v) = d^R_v(t(u^i_v))$. This can be verified using Lemma \ref{triv_lemma}(b).



\subsection{Proof of Proposition \ref{inherit_siggers}}




==> siggers.tex <==
Before giving proofs of Theorems \ref{coloreffective}, \ref{bjkineffective} and \ref{vcspconsineff},
we establish some basic facts about Siggers pairs that will be used in the proofs.

\begin{lemma}
Let $\Gamma$ be a crisp language on domain $D$ that admits a Siggers pair $(g,s)$ with $A\!=\!g(D)\!\subseteq\! D$. \\
(a) Language $\langle\Gamma\rangle$ also admits the Siggers pair $(g,s)$. \\
(b) Suppose that $\langle\Gamma\rangle$ contains a unary relation $B\subseteq D$.
Then $g(B)\subseteq B$ and $s(B\cap A, \ldots,  B\cap A)\subseteq B\cap A$.
\label{lemma:SiggersPairs}
\end{lemma}
\begin{proof}
\noindent {\bf Part (a)~~}
We need to show the following for every crisp function $f\in\langle\Gamma\rangle$ of arity $k=\ar(f)$:
(i) $f$ admits $g$; (ii) $f_{|A}$ (the restriction of $f$ to $A^{k}$) admits $s$.
The first claim holds by Lemma~\ref{lem:exppower}(a). We will show that $f_{|A}\in\langle\Gamma[A]\rangle$,
then the second claim will again follow by Lemma~\ref{lem:exppower}(a).

Since $f\in\langle\Gamma\rangle$, there exists a $\Gamma$-instance $\calI$ with $n\ge k$ variables such that
$$
f(\bx)=\min_{\by\in D^{n-k}} f_\calI(\bx,\by) \qquad \forall \bx \in D^k
$$
Define function $f':A^k\rightarrow\{0,\infty\}$ via
$$
f'(\bx)=\min_{\by\in A^{n-k}} f_\calI(\bx,\by) \qquad \forall \bx \in A^k
$$
By construction, $f'\in\langle\Gamma[A]\rangle$. It thus suffices to prove that $f_{|A}=f'$.
Consider $\bx\in A^k$. Clearly, we have $f(\bx)\le f'(\bx)$ (or equivalenty
$\bx\in \dom f'$ implies $\bx\in\dom f$). Suppose that $\bx\in \dom f$.
Then there exists $\by\in D^{n-k}$ such that $(\bx,\by)\in \dom f_{\calI}$.
Since $g$ is a polymorphism of $f_\calI$, we obtain $(g(\bx),g(\by))\in \dom f_{\calI}$.
The properties of $g$ stated in Definition~\ref{def:SiggersPair} and the fact $x\in A^k$
give that $g(\bx)=\bx$ and $g(\by)\in A^{n-k}$.
Therefore, $(\bx,\by')\in\dom f_{\calI}$ for some $\by'\in A^{n-k}$ and so $\bx\in\dom f'$.

 
\vspace{4pt}


\noindent {\bf Part (b)~~} The first claim holds since $A$ admits $g$.
We have $B\in\langle\Gamma\rangle$, and $B\cap A$ is the restriction of $B$ to $A$;
as we just showed, $B\cap A\in\langle\Gamma[A]\rangle$. Since $s$ is a polymorphism of language $\Gamma[A]$,
it is also a polymorphism of relation $B\cap A$. This implies the second claim.
\end{proof}


